Client-side Gradient Inversion Against Federated Learning from Poisoning

Federated Learning (FL) enables distributed participants (e.g., mobile devices) to train a global model without sharing data directly to a central server. Recent studies have revealed that FL is vulnerable to gradient inversion attack (GIA), which aims to reconstruct the original training samples and poses high risk against the privacy of clients in FL. However, most existing GIAs necessitate control over the server and rely on strong prior knowledge including batch normalization and data distribution information. In this work, we propose Client-side poisoning Gradient Inversion (CGI), which is a novel attack method that can be launched from clients. For the first time, we show the feasibility of a client-side adversary with limited knowledge being able to recover the training samples from the aggregated global model. We take a distinct approach in which the adversary utilizes a malicious model that amplifies the loss of a specific targeted class of interest. When honest clients employ the poisoned global model, the gradients of samples belonging to the targeted class are magnified, making them the dominant factor in the aggregated update. This enables the adversary to effectively reconstruct the private input belonging to other clients using the aggregated update. In addition, our CGI also features its ability to remain stealthy against Byzantine-robust aggregation rules (AGRs). By optimizing malicious updates and blending benign updates with a malicious replacement vector, our method remains undetected by these defense mechanisms. To evaluate the performance of CGI, we conduct experiments on various benchmark datasets, considering representative Byzantine-robust AGRs, and exploring diverse FL settings with different levels of adversary knowledge about the data. Our results demonstrate that CGI consistently and successfully extracts training input in all tested scenarios.

==> chapters/approach.tex <==
\section{Method}
In this section, we will introduce the entire framework of CTGI.  With the framework, the malicious clients controlled by the adversary can replace the global model with the malicious poisoning model and invert other benign clients' gradients to gain target data.

\subsection{Setting}
\lyz{Consider moving the whole sub-section to a new section by refer to some well-known papers.}

\subsubsection{Environment Setting}
We assume the adversary can control some malicious clients in a common federated learning system and the system based on \textit{FedSGD}~\cite{shokri_privacy-preserving_2015}. The system tries to train an image classifier(we focus on images) on a multi-class data distribution (i.e. class number $>$ 100). And the server has some general defence methods like \textit{robust aggregation algorithm} (AGR). Each client can get the global model in each round and some necessary training information from the server.


\subsubsection{Adversary’s Goal}
The adversary's goal is to gain other users' target class data. Specifically, the adversary first plays as a benign participator and joins training normally until the global model converges. Then he will download the global model and make a malicious replacement model, the model has the lowest accuracy on the target class but perform normally on other classes. After that, the adversary uses the malicious model to replace the global model and break robust aggregation. When the replacement step is finished, the adversary will use global models from each round to calculate other clients' gradients. Finally, the adversary can invert these gradients to get target class data. 


\subsubsection{Adversary’s Capabilities} 
We assume that the adversary controls m out of total N clients, called \textit{malicious clients}. And we assume the number of malicious clients is no more than 20\% in all adversarial setups, i.e., (m/N)$<$0.2. The attacker can download the global model of each round and directly manipulate local model updates of malicious clients.


\subsubsection{Adversary’s Knowledge}
We consider different adversary knowledge levels.
%Review%
The adversary has two knowledge dimensions: knowledge of current data distribution and knowledge of the AGR algorithm of the server. 
For knowledge of data distribution, we consider three levels: i) Full knowledge: the adversary has enough samples which cover the entire data distribution; ii) Semi-Target Knowledge: the adversary has few target samples and some other class samples (not necessary to cover all classes); iii) None-Target Knowledge: the adversary just knows some or full other class samples, but nothing about the target class.
With different knowledge levels, the adversary can choose different methods to make a malicious replacement model.
%Review%
About AGR,  we assume the adversary has no idea about the AGR. Different AGR not only affects model replacement processing but also makes gradient inversion harder. 

\subsection{Attack Framework} \label{section-framework}
In this subsection, we will show our general attack framework which includes three steps: making malicious models, replacing the global model, and finally to invert other users' gradients. 


\subsubsection{Intuition} 
According to some recent work~\cite{wen_fishing_2022,geiping_inverting_2020}, we find gradient inversion based on the averaged gradient from samples if one sample has a relatively large gradient which can overlook other small gradients from other samples. And the averaged gradient can be regarded as the target sample gradient. \lyz{Why?} This is easy to invert based on present methods. Thus, in FL, we can control some malicious clients to replace the global model, which may make the gradient of the target class sample obviously different from gradients from other class samples. When getting gradients including the target class gradient, it is possible to invert it. \lyz{Can we have a visualization here? Like there are n-1 class being trained to almost converge at time t-1, and then samples of one  new class just joined the training at time t? Will this make the intuition better explained?}


Let $\Phi$ denote the parameters of a DNN model and $\mathcal{L}$ denote the loss function. Furthermore,the batch size is $k$, $X = \{x_i\}_{i=1}^k; Y = \{y_i\}_{i=1}^k$, $(X,Y)$ represents any batch data, so we have gradient $g$:
$$g = \frac{1}{k}\sum_{i=1}^k\nabla_{\Phi}\mathcal{L}((x_i,y_i),\Phi)$$
If we have a target sample $x_t$, and the gradient of the loss with respect to parameters on $x_t$ is far larger than the gradient on other samples in the same batch, we have:
\begin{equation*}
\nabla_{\Phi}\mathcal{L}((x_t,y_t),\Phi) \gg \sum_{i\neq t}\nabla_{\Phi}\mathcal{L}((x_i,y_i),\Phi).  
\end{equation*}
Then the gradient $g$ of loss $\mathcal{L}$ w.r.t model parameters on batch data is:
$$g \approx \frac{1}{k} \nabla_{\Phi}\mathcal{L}((x_t,y_t),\Phi)$$

Now we assume these target sample $X_t$ belongs to the target class $Y_t$, so the problem is how to make the target gradient far larger than normal gradients:
$$\arg\max\limits_{\Phi}\nabla_{\Phi}\mathcal{L}((X_t,Y_t),\Phi) - \sum_{c\neq t}\nabla_{\Phi}\mathcal{L}((X_c,Y_c),\Phi)$$
where $c$ is the class label. \lyz{$\arg\max_x f(x)$ returns $x$ but not $\max f(x)$. }


Considering the formula, we know that when maximizing loss $\mathcal{L}$, the gradient $\nabla_{\Phi}\mathcal{L}((X,Y),\Phi)$ also increases \lyz{(Not always correct since $\max f(x)$ has zero gradient at its maximum.)}, so we get:

\begin{equation}
\begin{aligned}
    & \arg\min\limits_{\Phi} \mathcal{L}((X_c,Y_c),\Phi) \\
    & \arg\max\limits_{\Phi} \mathcal{L}((X_t,Y_t),\Phi)
    \label{eq1}
\end{aligned}
\end{equation}
where $c\neq t$. 


Finally, we find what we need is a target poisoning model or known as \textit{targeted model poisoning attack}


\subsubsection{General Framework} As an adversary in FL, he can control malicious clients and have some knowledge about data distribution. Firstly, the adversary plays as a benign member and makes a small validation dataset $\mathcal{D}_{aux}^{val}$. He can gain the global model $\Phi_G$ in each round and check if the global model converged with the validation dataset. If the global model converged in adversary view ($\mathcal{L}(\mathcal{D}_{aux}^{val},\Phi_G)$ does not change in multi-round), he will download $\Phi_G$ and try to make a target poisoning model $\Phi_{rep}$ as malicious replacement model to replace global model $\Phi_G$. According to the distribution knowledge of the adversary, he can use different functions $f_{poi}$ to make the target poisoning model. The methods include  \textbf{model retraining},\textbf{model poisoning}, and \textbf{model inversion poisoning}. Then the adversary get $\Phi_{rep} = f_{poi}(\Phi_G,\mathcal{D}_{aux})$. The replacement model $\Phi_{rep}$ performs normally on almost classes but fails on the target class. The next step is to replace the global model $\Phi_{G}$ and break robust aggregation. The adversary tries to craft a malicious update $\delta_m$. In CTGI, 
%Review%
the adversary chooses the perturbation vector $\nabla^p$ and optimizes it with the benign updates $\overline{\delta}_{ben}$ that malicious clients can produce to approach the aggregation update $\delta_{agr}$. Now the adversary has the malicious update $\delta_m = f_{attack}(\delta_{agr},\Phi_{rep},\overline{\delta}_{ben},\nabla^p)$. He can produce and submit the malicious update in multiple training rounds until the global model has been replaced.
%Review%%Review%
The final step is to invert gradients from other benign clients. To gain the aggregation gradient $\delta_{agr}^{t-1} = f_{rec}(\Phi_G^{t-1} - \Phi_G^{t})$, if current training round contains a target class sample, its gradient would dominate the benign gradients. Then the adversary will get other participators' privacy data of target class: $X_{tar} = f_{inv}(\delta_{agr}^{t-1},\Phi_G^{t-1},Y_{tar})$. \lyz{(It is not clear for me as there are too many new symbols, can we (partially) associate this process with Fig.~1?)}


\subsection{Malicious Model} \label{section-maliciousModel}
\lyz{(This is already somehow included in Sec. 3.1.4, so a better organisation is needed. Otherwise, it is chaotic.)}

Considering the complex environment in federated learning and its stable effect, we will create the malicious replacement model locally. Here, we discuss some possible and heuristic methods to craft a malicious replacement model based on different knowledge levels of the adversary.

\subsubsection{Full knowledge - Model retraining}
If the adversary has full knowledge of the entire data distribution, he can craft two datasets:
\begin{equation}
\begin{aligned}
& D_{aux} = \{(x_i,y_i)\} \\
& D_{trap} = \{(x_i,y_{tar})\} \\
& D_{aux} \cap D_{tar} = \emptyset \\
\end{aligned}
\end{equation}
where $D_{aux}$ is the auxiliary dataset covering the entire data distribution but the target class, $D_{tar}$ is the dataset that only contains target class data and $D_{trap}$ is the special dataset that consists of samples from $D_{aux}$ but labeled by target class $y_{tar}$.

Then with $D_{aux}$, the adversary actually can retrain a malicious replacement model without target class data then naturally the model cannot recognize the target class.  At the same time, the malicious replacement model must achieve a large gap performance between the target class and other classes, which requires increasing the loss of $D_{trap}$ on the replacement model.

\begin{equation}
\begin{aligned}
& \Phi_{rep}^{t+1} = \Phi_{rep}^t - \alpha_{1}\nabla_{\Phi_{rep}^t}\mathcal{L}(\Phi_{rep}^t,D_{aux}) \\
&\Phi_{rep}^{t+1} = \Phi_{rep}^t + \alpha_{2}\nabla_{\Phi_{rep}^t}\mathcal{L}(\Phi_{rep}^t,D_{trap}) \\
% & \arg\min\limits_{\Phi_{rep}}\mathcal{L}(\Phi_{rep},D_{aux}) \\
% & \arg\max\limits_{\Phi_{rep}}\mathcal{L}(\Phi_{rep},D_{trap})
\end{aligned}
\end{equation}

where $\Phi_{rep}$ is the malicious replacement model parameters.

\subsubsection{Semi-Target knowledge - Model poisoning}
%Review%%Check Data Augmentation%
Under this condition, the adversary only has few target samples. We think the simplest poisoning method~\cite{munoz-gonzalez_towards_2017} is an effective choice. He can download the converged global model first, then calculate the gradient of loss on these target samples with respect to the weights of the model, and finally, reduce the gradient from the weights of model in each round.
%Review%
\begin{equation}
\begin{aligned}
%& D_{aux} \cap D_{tar} = \emptyset \\%
\Phi_{rep}^{t+1} = \Phi_{rep}^t + \alpha_1\nabla_{\Phi_{rep}^t}\mathcal{L}(\Phi_{rep}^t,D_{tar})
\end{aligned}
\end{equation}

where $\alpha_1$ is the learning rate and $D_{tar}$ is the crafted dataset only including target class samples, $t$ is the index of round, when $t=0$, $\Phi_{rep}^0 = \Phi_G$. 

But sometimes, the lost features will damage model generalization on other classes. So the adversary still needs a $D_{aux}$ which is used to repair cross-class common features.
\begin{equation}
\begin{aligned}
%& D_{aux} \cap D_{tar} = \emptyset \\%
\Phi_{rep}^{t+1} = \Phi_{rep}^t -\alpha_2\nabla_{\Phi_{rep}^t}\mathcal{L}(\Phi_{rep}^t,D_{aux})
\end{aligned}
\end{equation}
generally, the repair and poisoning processes are alternating. It can keep the main task accuracy as target class loss increases.

\subsubsection{None-Target knowledge - Model inversion poisoning} The least knowledge level is the adversary has no samples of the target class but still has some other class samples as a normal participator. In this case, the adversary can try to craft some target samples by model inversion methods and then to follow model poisoning.
% \yanjun{Would the malicious model of ``None-Target knowledge'' require the knowledge of the data distribution of non-victim classes (the classes that are not under attack) to simulate $D_{aux}$?}
% \jiaheng{Yes. But just samples from some classes, it's not necessary to cover all distribution.}

Model inversion poisoning combined model inversion~\cite{fredrikson_model_2015,ye_model_2022,yin_dreaming_2020} and model poisoning~\cite{munoz-gonzalez_towards_2017}. The first step is to invert the model to gain target class knowledge, here we mainly referenced \textit{DeepInversion}~\cite{yin_dreaming_2020}. Thus the model inversion method is like this:
\begin{equation}
\begin{aligned}
\hat{X}_{tar} = \arg\min\limits_{\hat{X}}& \ \lambda_0 \mathcal{L}(\Phi_G,(\hat{X},Y_{tar})) 
\\ 
&+ \lambda_1 \mathcal{R}_{TV}(\hat{X}) 
\\ 
&+\lambda_2 \mathcal{R}_{l_2}(\hat{X})
\\ 
&+\lambda_3 \mathcal{R}_{f}(\hat{X})
\end{aligned}
\end{equation}

where $\hat{X}_{tar}$ represents reconstructed samples of target class,$Y_{tar}$ is the target class label array, $\lambda$ is the coefficient $\mathcal{R}_{TV}$ and $\mathcal{R}_{l_2}$ are regular items of total variation and $l_2$ norm. $R_f$ is used to optimize feature similarities according to statistic values of mean $\mu$ and variance $\sigma^2$. 

\begin{equation}
\begin{aligned}
R_{f}(\hat{X}) & = \sum\limits_l||\mu_l(\hat{X})-BN_l(mean)||_2 \\
&+ \sum\limits_l||\sigma^2_l(\hat{X})-BN_l(variance)||_2
\end{aligned}
\end{equation}

where $l$ represents the $l^{th}$ batch normalization layer. In federated learning, if the model structure contains batch normalization layers, the adversary as a normal participator can easily gain the mean and variance from the global model. With statistic values, \textit{DeepInversion} attack can produce better target class data.

Then the adversary can use knowledge of the target class data to poison the model and let it have a higher loss on the target class. 

\begin{equation}
\begin{aligned}
&\hat{D}_{tar} = \{(x,y)|x\in \hat{X}_{tar}, y \in Y_{tar}\}
%D_{aux} \cap D_{tar} = \emptyset %
\\
&\Phi_{rep}^{t+1} = \Phi_{rep}^t + \alpha_1\nabla_{\Phi_{rep}^t}\mathcal{L}(\Phi_{rep}^t,\hat{D}_{tar})
\end{aligned}
\end{equation}

$\hat{D}_{tar}$ is the crafted dataset only including target class samples, $t$ is the index of round, when $t=0$, $\Phi_{rep}^0 = \Phi_G$.

Similarly, the MIP method also requires model generalization repair. Thus, malicious clients can use their own datasets without target class samples to make the $D_{aux}$ and use it to resume lost common features.
\begin{equation}
\begin{aligned}
%& D_{aux} \cap D_{tar} = \emptyset \\%
\Phi_{rep}^{t+1} = \Phi_{rep}^t -\alpha_2\nabla_{\Phi_{rep}^t}\mathcal{L}(\Phi_{rep}^t,D_{aux})
\end{aligned}
\end{equation}


% \noindent
% \textbf{Method 2. Machine unlearning} \\
% Machine unlearning\cite{bourtoule_machine_2021}\cite{sekhari_remember_2021} is a kind of new technology which help model forget some learned knowledge based on law or users' requirements. Machine unlearning generally has two objectives: to unlearn some data points\cite{cao_towards_2015} or to forget some learned class information\cite{tarun_fast_2022}. Here, the adversary based on the later objective tries to make the model unlearn the target class. And we reference the method from\cite{tarun_fast_2022}. The adversary can maximize the loss of reconstructed samples on the target class, then he gets the most dissimilar target class samples. When feeding these adversarial samples with target class labels to the model, the model will forget the target class but it may also cause lower performance on other classes. Thus, the final step is to use the auxiliary dataset to repair model generalization.~\yanjun{It seems that only machine unlearning requires the step of repair. (1) Just wondering whether others such as model poisoning and model inversion+poisoning also reduce the performance on other classes as well? (2) Would the repair affect the performance on the target class? }
% \jiaheng{(1) Yes. Target class images contain natural image features and unique class features, to reduce the gradient of target class images damaged learned natural image features which reduce the performance on other classes. (2) Perhaps a little or None. For the unique class features have lost, only natural image features cannot help target class performance}

% \begin{equation}
% \begin{aligned}
% X_{atar} &= \arg\min\limits_{\hat{X}} -\mathcal{L}(\Phi_G,(\hat{X},Y_{tar})) \\
% &+ \lambda_1 \mathcal{R}_{TV}(\hat{X}) \\
% &+\lambda_2 \mathcal{R}_{l_2}(\hat{X})
% \end{aligned}
% \end{equation}

% \begin{equation}
% \begin{aligned}
% & D_{atar} = \{(x,y)|x\in X_{atar}, y \in Y_{tar}\}
% \\
% %D_{aux} \cap D_{tar} = \emptyset %
% &\Phi_{rep}^{t_0+1} = \Phi_{rep}^{t_0} - \alpha\nabla_{\Phi_{rep}^{t_0}}\mathcal{L}(\Phi_{rep}^{t_0},D_{atar})
% \\
% &\Phi_{rep}^{t_1+1} = \Phi_{rep}^{t_1} - \alpha\nabla_{\Phi_{rep}^{t_1}}\mathcal{L}(\Phi_{rep}^{t_1},D_{aux})
% \nonumber
% \end{aligned}
% \end{equation}

% where $\hat{X}_{atar}$ represents adversarial samples of target class,$Y_{tar}$ is the target class label array, $\mathcal{R}_{TV}$ and $\mathcal{R}_{l_2}$ are regular items of total variation and $l_2$ norm, $\lambda$ is the coefficient, $D_{atar}$ is the adversarial dataset containing adversarial target class samples,$D_{aux}$ is the auxiliary dataset. $t_0$ is the index of unlearning round, $t_1$ represents the index of repair round, when $t_0=0$, $\Phi_{rep}^{t_0} = \Phi_G$.


\subsection{Model Replacement} \label{section-modelReplacement}
In this section, we will show how to replace the global model with the crafted malicious target poisoning model.


\subsubsection{Intuition}
% Following proposed AGRs, we found almost robust AGRs for FL tend to remove malicious updates based on such criteria: i) distances from benign gradient: \textit{Krum, Multi-Krum}\cite{blanchard_machine_2017}, \textit{Bulyan}\cite{mhamdi_hidden_2018} ii)cosine similarity from benign gradient: \textit{Adaptive federated average(AFA)}\cite{cao_fltrust_2022} iii) distributional bias with the benign gradients: \textit{Trimmed-mean},\textit{Median}\cite{xie_generalized_2018} \cite{yin_byzantine-robust_2018} iv) loss and error differences: \textit{Fang}\cite{fang_local_2020}.
%review Median, Trimmed-mean%
%review Krum%
Following existing and popular AGRs, we mainly focus on \textit{Multi-Krum}~\cite{blanchard_machine_2017},\textit{Bulyan}~\cite{mhamdi_hidden_2018},\textit{Adaptive federated average (AFA)}~\cite{cao_fltrust_2022} and \textit{Fang}~\cite{fang_local_2020}. For these AGRs still, calculate the average gradient after filtering malicious gradients. \textit{Trimmed-mean} and \textit{Median}~\cite{xie_generalized_2018,yin_byzantine-robust_2018} aggregate gradients according to sorted gradient values in each dimension, which is far from our core theory. Thus, our attack framework on  \textit{Trimmed-mean} and \textit{Median} is inapplicable.
We define the replacement problem as below:

\begin{equation}
\begin{aligned}
& \delta_i = \nabla_{\Phi_i}\mathcal{L}(D_i)
\\
& \delta_{agr} = f_{AGR}(\delta_{\{i\in[m]\}}\cup\delta_{\{i\in[m+1,N]\}})
\\
& \delta_{rep} = ||\Phi_G-\Phi_{rep}||_2
\\
& \arg\min\limits_{\delta_{\{i\in[m]\}}} f_{dis}(\delta_{agr},\delta_{rep})
\end{aligned}
\end{equation}

where $\delta_i$ represents the gradient update from client $i$, $\delta_{rep}$ is the distance of weights between global model $\Phi_G$ and malicious replacement model $\Phi_{rep}$, and $\delta_{agr}$ is the aggregation gradient from last round. Here, we tend to minimize a distance function $f_{dis}$ between $\delta_{rep}$ and $\delta_{agr}$. If no AGR, the adversary can directly commit $\delta_{rep}$ as $\delta_m$.


\subsubsection{Method} But the above formula is hard to optimize for the uncertainty of AGRs, and our \textit{targeted model poisoning attack} is between untargeted model poisoning attack and backdoor attack. After referencing related attacks~\cite{fang_local_2020,shejwalkar_manipulating_2021,bhagoji_analyzing_2019}, we proposed our attack and it is universal for all AGRs:

\begin{equation}
\begin{aligned}
&\nabla^p = \gamma\frac{\delta_{rep}}{||\delta_{rep}||}
\\
&  \delta_m = \nabla^p + \beta \overline{\delta}_{ben}
\\
& \delta_{agr}^{t-1} = \frac{1}{\alpha}(\Phi_G^{t-1} - \Phi_G^t)
\\
& \arg\min\limits_{\gamma,\beta}||\delta_{m}^t - \delta_{agr}^{t-1}||_2
\end{aligned}
\end{equation}

where $\nabla^p$ is the perturbation vector that equals the unit vector of replacement distance $\delta_{rep}$, $\gamma$,$\beta$ are the scaling coefficients for the malicious unit gradient and reference gradient. And the initialized value $\gamma_0$ and $\beta_0$ are two tunable hyper-parameters that can decide the poisoning amount. $\delta_{agr}^{t-1}$ is the aggregation gradient in round $t-1$ which is calculated by differences between model weights updates and $\alpha$ is the learning rate of the server (we assume the server optimize model with SGD). In the current attack, all malicious clients can also compute their benign gradients with their auxiliary dataset, $\overline{\delta}_{ben}$ represents the average of benign gradients from malicious clients. Then, the adversary tends to optimize $\gamma$,$\beta$ and minimize the distance between malicious update $\delta_m^t$ in round $t$ and aggregation gradient $\delta_{agr}^{t-1}$ in round $t-1$ to break AGRs. And the adversary will make all the malicious clients submit the same gradients.

\subsection{Gradient Inversion} \label{section-gradientInversion}
In this section, we will demonstrate how to invert other benign gradients from the client side.

\subsubsection{Gain Target Gradient}
Actually, the adversary as the client side only obverses the aggregation gradient:
$$\delta_{aggregation}^{t-1} = \frac{1}{\alpha}(\Phi_G^{t-1} - \Phi_G^t)$$

But for different AGRs, the aggregation gradient cannot be regarded as the average of all commit gradients:
$$f_{agr}(\delta_{\{i\in[N]\}}) \neq \frac{1}{N}\sum\limits_{i=1}^N \delta_{i}$$


Some malicious gradients will be removed before aggregation, and in CTGI, the gradients including target class samples (target gradient) show obvious differences from other benign gradients, which makes target gradients easier identified as malicious gradients. The adversary cannot control benign gradients and normal clients, but in a practical case, if the number of target gradients is more than other benign gradients and selected in the remaining set, our attack still can operate  for almost AGRs will averagely aggregate the remaining gradient set:
\begin{equation}
\begin{aligned}
& \delta_{\{i\in\{S\}\}}^{t-1} = f_{agr\_select}(\delta_{\{i\in[N]\}}^{t-1})
\\
& \frac{1}{|S|}\sum\limits_{i=1}^{|S|} \delta_{i}^{t-1} = f_{agr\_aggregate}(\delta_{\{i\in[S]\}}^{t-1})
\\
& \delta_{aggregation}^{t-1} =\frac{1}{|S|}\sum\limits_{i=1}^{|S|} \delta_{i}^{t-1}
\\
&\delta_{aggregation}^{t-1} = \frac{1}{\alpha}(\Phi_G^{t-1} - \Phi_G^t)
\end{aligned}
\end{equation}
% \yanjun{A bit confused about the above equations, need to discuss.}
where $S$ is the remaining gradient set, the adversary can get the aggregation gradient through the differences between model weights. If the aggregation gradient contains the target gradient, the adversary now can invert it. 

\subsubsection{Gradient Inversion Method}
We chose the optimization way as our main gradient inversion method. Basically,  the optimization is based on distance~\cite{zhu_deep_2019} or cosine similarity~\cite{geiping_inverting_2020}. Considering the aggregation contains other samples gradients, here we directly referenced InV~\cite{geiping_inverting_2020} and chose cosine similarity as criteria to design our inversion method:
\begin{equation}
\begin{aligned}
\delta_{tar} & = \nabla_{\Phi_G^{t-1}}\mathcal{L}(\hat{X}_{tar},\hat{Y}_{tar})
\\
\arg\min\limits_{\hat{X}_{tar}} &\lambda_0 (1-\frac{<\delta_{tar},\delta_{aggregation}^{t-1}>}{||\delta_{tar}||||\delta_{aggregation}^{t-1}||})
\\
&+ \lambda_1 R_{TV}(\hat{X}_{tar})
\\
&+ \lambda_2 R_{l_2}(\hat{X}_{tar})
\\
&+ \lambda_3 R_{clip}(\hat{X}_{tar})
\end{aligned}
\end{equation}

where $\hat{X}_{tar}$ is the reconstruction data, $\hat{Y}_{tar}$ is the target label array. we will set the length of $\hat{X}_{tar}$ according to the probability of target class samples in the aggregation gradient, generally, we set $|\hat{X}_{tar}|$ with a small value like $1$ or $2$. Then, we tend to optimize $\delta_{tar}$ to approach $\delta_{aggregation}^{t-1}$, $\lambda$s are coefficients, $R_{TV}$,$R_{l_2}$ and $R_{clip}$ are the total variation item, the $l_2$ norm item and the clip item. $R_{clip}(\hat{X}_{tar}) = ||f_{clip}(\hat{X}_{tar},[0,1])-\hat{X}_{tar}||_2$
% \yanjun{(1) What is $\hat{Y}_{tar}$, as previously it's ${Y}_{tar}$? (2) What is the length of $\hat{X}_{tar}$? The number of inverse samples?} \jiaheng{(1)Yes. (2)1 or 2, according to our core theory: the target class sample gradient is larger than other class gradients, if we have more target class samples, target class sample gradients will disturb each other, thus we hope the number of inverse samples is small.}

==> chapters/discussion.tex <==
\section{Discussion}
\subsection{Evaluation of CTGI}
\subsubsection{Comparison with the state-of-the-art gradient inversion attacks} According to existing attacks~\cite{zhu_deep_2019,geiping_inverting_2020,zhao_idlg_2020,yin_see_2021,boenisch_when_2021,wen_fishing_2022,fowl_robbing_2022,jeon_gradient_2021,karras_analyzing_2020,usynin_beyond_2022}, CTGI is the first kind of gradient inversion attack based on optimization that can be launched from the client side and gain other clients' privacy data in the federated learning framework. In section~\ref{section-literature-inversionattck}, we find that in all existing gradient inversion attacks, the adversary has to invert gradients locally or be a server in federated learning. In Figure~\ref{fig:CompGradInversion}, we compare our method with DLG~\cite{zhu_deep_2019},iDLG~\cite{zhao_idlg_2020} and IG~\cite{geiping_inverting_2020} that only our method can invert target sample successfully from the client side. Next, we give the advantages of our method compared to other methods.



\paragraph{Client-Side Attack}  The main highlight of our method is that the adversary can gain other clients' private data as a general client. For DLG~\cite{zhu_deep_2019} and IG~\cite{geiping_inverting_2020}, the two methods cannot work well in a realistic environment with a large batch size and plenty of clients. GradInversion~\cite{yin_see_2021} mainly relies on the batch normalization layer information, if as a client, such information cannot be captured under the normal training framework. Other methods~\cite{boenisch_when_2021,wen_fishing_2022,fowl_robbing_2022} change the general federated learning framework. They either need to send malicious models to clients or modify the training structure on the server side. But for our method, the adversary plays as a client and does not break the general training framework. If the number of categories is large, the attack can be stealthy. Moreover, our attack is targeted, which can tolerate more noise and work in a more realistic environment.

\paragraph{No Label Restoration} For gradient inversion attacks based on optimization, better label restoration can obviously enhance inversion attacks. In related work, iDLG~\cite{zhao_idlg_2020} can find the true label of a single image according to the gradient of the last layer based on cross-entropy loss. Then GradInversion~\cite{yin_see_2021} proposed a batch label restoration method, but it cannot handle the condition that one batch contains two or more same labels. In our method, considering the large batch size and plenty of clients, restoring all labels is hard and unnecessary. Thus, we try a targeted method, and the adversary generally focuses on some special classes rather than the entire data distribution.

\paragraph{Low Prior Knowledge Requirement} Comparing with generative methods~\cite{jeon_gradient_2021,karras_analyzing_2020,usynin_beyond_2022}, our method does not require strong prior knowledge, and we provide three methods for the different knowledge levels. Our attack totally follows the normal framework and does not require more information than normal clients.


\paragraph{Inversion Ability}
In our opinion, the theoretical inversion ability of our method depends on the used dataset or data and the number of other images determined by the batch size and client number. In the practical environment, the quality of malicious models and the final target model replacement distance also affect inversion ability. For AGRs, different AGR changes the number of gradients that joined the final aggregation and the difficulty of model replacement. But only if any AGR used standard aggregation in the final step, our attack can still work. 

\subsubsection{Comparing different malicious models}
About how to craft malicious models, we proposed three methods: model retraining (MR), model poisoning (MP), and model inversion poisoning (MIP). We will compare the three different malicious models on precondition, model replacement, and inversion performance.

\paragraph{Precondition} Considering prior knowledge requirement, MR needs full knowledge of the entire distribution of data, but compared with the other two methods, MR does not require the converged global model. The core method of MP and MIP is model poisoning. Thus, the converged global model is necessary. MP and MIP both need target class samples, but MIP can extract target class knowledge from the global model. In the three methods, MIP has no requirement for prior knowledge, but it spends more computation resources and has uncertainty depending on the quality of the extracted target knowledge.





\paragraph{Model Replacement} The most important factor is AGR at this stage. In our experiment, AFA~\cite{cao_fltrust_2022} and Fang~\cite{fang_local_2020} are more robust than the other two AGRs because the validation dataset can detect some malicious gradients, and if the validation data is all target class data, the replacement is very hard. According to Table~\ref{Table_ModelRep}, MP is the easiest one to replace the global model for it has the shortest replacement distance and works well in the main task. Oppositely, MR works difficultly in model replacement. For when MR increases target class loss, it also magnifies the main task loss, which makes it easier to be refused by AGR, and the too-long replacement distance becomes another reason. Then for MIP, the effectiveness of model replacement falls in between. 

\paragraph{Inversion Performance}
 Generally, if we have enough prior knowledge and can select any malicious model, we will care more about which malicious model can work under larger federated learning frameworks and can gain images with better quality. So, we use the same setting and the same input to compare different malicious models on three selected datasets. The result has been given in Figure~\ref{fig:ModelComparison}. We can see MR has the best performance on image quality and can work under a larger federated learning framework. MIP can work with more clients compared to MP. But MIP and MP performance are unstable.

% \begin{figure}[!t]
% \centering
% \includegraphics[width=0.5\textwidth]{Figure/Comparison of models.jpg}
% \caption{Comparison of models' inversion performance. The values under the setting represent the number of clients and batch size.}
% \label{Fig_ComparisonOfModels}
% \end{figure}



\subsection{Inversion Probability}
In this subsection, we will discuss the inversion probability under our attack. We assume that samples of each class have the same probability drawn from the data distribution. In the data distribution, we have $n$ classes, so the probability of each sample belonging to the target class is $\frac{1}{n}$. In training, a batch has $k$ samples, and the number of clients is $N$. Thus, the probability of one or more target samples appearing in one training round is: 
\begin{equation}
P_{target} = 1-((\frac{n-1}{n})^k)^N
\end{equation}
If AGR is just to average all gradients, the best condition is only one target sample in aggregation, the probability is:
\begin{equation}
P_{best} = (\frac{1}{n}\times(\frac{n-1}{n})^{k-1})\times((\frac{n-1}{n})^k)^{N-1}
\end{equation}
If we consider robust AGRs and all gradients that include target samples will be removed, the optimal condition of one round for our attack is only one target sample in the final selected set $S$, and the AGR filters $N-|S|$ gradients. The probability is:

\begin{equation}
\begin{aligned}
 P_{best-agr} = &(1-(\frac{n-1}{n})^k)^{N-|S|} \\
 \times
 &(\frac{1}{n}\times(\frac{n-1}{n})^{k-1}) \\
 \times
 &((\frac{n-1}{n})^k)^{|S|-1}
\end{aligned}
\end{equation}
Now, we assume the data distribution has $n=200$ classes, the FL framework contains $N=100$ clients and batch size is $k=128$. The probability of an optimal round for our inversion attack is $6.86\times10^{-31}$ under standard AGR and $9.94\times10^{-33}$ under robust AGR with $|S|=0.6N$. But if malicious clients just submit small updates to maintain the global model poisoning state, the probability now is $2.57\times10^{-25}$ and $3.72\times10^{-27}$ under robust AGR with $|S|=0.6N$. 

Surely, we also consider the non-best condition, which means more than one target image will appear in one round. We set 2 and 4 target images in one round. Besides, we also study the effect of target image distribution and assume two kinds of typical conditions: all target images come from a single client and target images are distributed averagely among multiple clients.
We set client 40 and batch size 32 with Multi-krum~\cite{blanchard_machine_2017} aggregation with TinyImageNet~\cite{tiny-imagenet} and malicious clients are 8. 

Figure~\ref{fig:MultiInversion} illustrates the inversion consequence. From the result, we verify our method can still work under the multiple target samples condition. But we observed semantic features transferring in multiple samples inversion. If target images are similar, the inversion algorithm will be confusing because it cannot identify which target image those semantic features belong to. Thus, the inverse target images will be more similar and averaged. Moreover, the target gradient with the largest loss may cover other target gradients. We believe this is also a reason for target feature transfer. Then, about target image distribution in clients, we can see that single-client distribution is more likely to cause image feature transfer because in the single client, target images aggregate earlier which reduces target feature independence. Briefly, CTGI still succeeds in multiple target image inversion.

\subsection{Effect of Framework Setting}~\label{section-discussion-setting}
\subsubsection{Effect of the Batch Size and the Number of Clients}~\label{subsection-batch-effect}
According to our core theory that our inversion attack succeeds when the target sample gradient dominates the averaged gradient, we can imagine there is an upbound if the batch size or the number of clients is very large. We know in one batch with size $k$, the batch gradient will be:
$\frac{1}{k}\sum_{i=1}^k\delta_i$. In FL, the standard aggregation gradient will be $\frac{1}{N}\sum_{c=1}^N\delta_c$ where $N$ represents the number of clients. Thus if one target sample appears in one client, we have $\delta_{agr} = \frac{1}{N}\frac{1}{k}(\sum_{c=1}^{N-1}\sum_{i=1}^k\delta_i + \sum_{i=1}^{k-1}\delta_i + \delta_{tar})$. If we want $\delta_{agr} \approx  \frac{1}{N}\frac{1}{k}\delta_{tar} $, We must guarantee
$\delta_{tar} - (\sum_{c=1}^{N-1}\sum_{i=1}^k\delta_i + \sum_{i=1}^{k-1}\delta_i)  > \mu$ where $\mu$ is the guarantee of our inversion attack. Then we can find if the batch size and the number of clients increases, the guarantee $\mu$ will fail. But we cannot directly point out the $\mu$ for different data distribution and training models.

Thus, we apply different settings on TinyImageNet~\cite{tiny-imagenet} with the MP method and standard aggregation. We use three metrics as the dependent variable to watch inversion performance. And use the image number as the independent variable according to the above discussion. The result has been given in Figure~\ref{fig:BatchEffectChart}. When the total image amount is small, the inversion effect is unstable because some values in the target class gradient are too large, increasing gradient variance and damaging the inversion effect. But if to increase the batch size or the number of clients, the target gradient will return to the reasonable gradient value range and be distinct compared to the general gradient on other samples. Then, depending on the previous discussion, we know as the batch size and the number of clients grow, malicious models will achieve their inversion ability upbound. And due to random images in the batch, some images may have a significant loss because of misclassification or underfitting, which perhaps influences inversion performance.



% \begin{figure*}[]
% \centering
% \includegraphics[width=1\textwidth]{Figure/Batch_Effect_Image.jpg}
% \caption{Inverse images under different settings. Applied PSNR, LPIPS, and SSIM as metrics}
% \label{Fig_BatchEffect}
% \end{figure*}


\subsubsection{Effect of AGR} According to our core theory, the success of our attack depends on the larger target gradient which can cover small values of other gradients, so our attack only applies to AGRs with averaging aggregation. And this is why \textit{Trimmed-mean}~\cite{xie_generalized_2018,yin_byzantine-robust_2018} and \textit{Median}~\cite{xie_generalized_2018,yin_byzantine-robust_2018} are not applicable for our attack. The two AGRs will choose the median value in the same element position of all submitted gradients, then the larger target gradient will be filtered out. 

For the entire attack framework, AGRs mainly act on the model replacement process and if replacement is ideal, they basically have no effect on the inverse image quality. But here AFA~\cite{cao_fltrust_2022} is a special case, for it uses weighted averaging aggregation which makes inversion performance unstable, but under almost all conditions our method still works on it.

\subsection{Effect of Loss Gap} 
The target of CTGI is to gain semantic private images from other clients. Therefore, we try to quantitatively analyze how the aggregated gradient impacts semantic image feature inversion. We know when the target gradient is further larger than other gradients, it will dominate the final aggregated gradient. But it is hard to directly compare the target gradient with general gradients. Due to the comparison based on numerical values, we choose the loss gap as the metric for the loss numerical value, which can determine gradient numerical values in the back-propagation.
We define the loss gap $L_{gap}$ as follows:
\begin{equation}
\begin{aligned}
& B = B_{gen} \cup B_{tar} \\
& B_{gen} = \{(x_i,y_i)|y_i\neq y_{tar}\} \\
& B_{tar} = \{(x_j,y_{tar})\} \\
& B_{gen} \cap B_{tar} = \emptyset \\
& L_{gen} = \mathcal{L}(\Phi,B_{gen}) \\ 
& L_{tar} = \mathcal{L}(\Phi,B_{tar}) \\ 
& L_{gap} = \frac{L_{tar}}{L_{tar}+L_{gen}}
\end{aligned}
\end{equation}
where $B$ is the current input batch, $B_{tar}$ is the subset of $B$ that only includes target samples, $B_{gen}$ contains the rest of general samples. $L_{gen}$ and $L_{tar}$ are two losses on $B_{gen}$ and $B_{tar}$ based on test model $\Phi$. And loss gap $L_{gap}$ represents the ratio of $L_{gen}$ to the entire batch loss.

To step-by-step control loss, we conduct the experiment on TinyImageNet~\cite{tiny-imagenet} under the setting of 40 clients and batch size 32 with the MR method. And we still use PSNR, LPIPS~\cite{zhang2018unreasonable}, and SSIM~\cite{wang2004image} to evaluate inverse image quality. Figure~\ref{fig:LossGapChart} demonstrates how the loss gap affects inverse image quality. When the loss gap is small,  the target gradient is not distinct and mixes other image features together. By increasing the loss gap, the target gradient will be distinct, and the inversion algorithm can easily make the dummy gradient approach the target gradient. Then, if we continue to enhance the loss gap, the target gradient will gradually dominate the aggregated gradient so the inversion performance increases. Finally, if the model can correctly identify each non-target image and the logits near batch labels, the loss will be zero, and according to back-propagation, the gradient values will also be zero. At that time, the aggregated gradient equals the target gradient. But this is an ideal condition and never happens. The above-detailed experiment of the loss gap can explain the principle of our method.








==> chapters/eval.tex <==
\section{Experiments}
In this section, we will conduct experiments to validate our method and show the attack performance. 

\subsection{Datasets and Model Architectures}
We apply our method on Cifar100~\cite{krizhevsky2009learning}, TinyImageNet~\cite{tiny-imagenet}, and CalTech256~\cite{griffin2007caltech}. We choose Resnet18~\cite{he2016deep} as our defeat model structure.

\noindent
\textbf{Cifar100}~\cite{krizhevsky2009learning} is a 100-class classification task dataset with 60000 RGB images. All images are 32 x 32. There are 500 training images and 100 testing images per class. 

\noindent
\textbf{TinyImageNet}~\cite{tiny-imagenet} is a subset of ImageNet. It contains 100000 images from 200 classes. Each image is a 64 x 64 coloured image. 

\noindent
\textbf{CalTech256}~\cite{griffin2007caltech} is an object recognition dataset containing 30,607 real-world images, of different sizes, spanning 257 classes. We scaled the images to 112 x 112 and selected 256 classes in our task. 

\subsection{FL setting}
We use XX clients and we set the number of malicious clients as 20\% in all adversarial setups, i.e., \highlight{(m/N)$<$0.2}~\yanjun{do we have experiments of various number of malicious clients?}

\subsection{Malicious Model Evaluation}
In the previous section~\ref{section-maliciousModel}, we introduce three methods: \textit{Model Retrain} (MR), \textit{Model Poisoning} (MP), and \textit{Model Inversion Poisoning} (MIP). We apply the three methods to each dataset and craft 9 malicious models.

\subsubsection{Implement Details}\label{subsection-maliciousmodelhyperparameters}
In crafting malicious models with MP and MIP methods, we use the overfitting global model, which has  been broadcast  to malicious clients. For the MR method, we use SGD as the optimizer and $\alpha_1 = 1\times10^{-2}$, $\alpha_2 = 1\times10^{-5}$ for all datasets and we run 30 iterations on  \textit{Cifar100}, \textit{TinyImageNet}, then 15 epochs on \textit{CalTech256}. In the MP method,  $\alpha_1 = 5\times10^{-3}$ for all datasets in the poisoning process. Then to avoid overfitting on auxiliary datasets, we use a small learning rate for the repair step. We set $\alpha_2 = 1\times10^{-4}, 1\times10^{-4}, 1\times10^{-5}$ for \textit{Cifar100}, \textit{TinyImageNet}, and \textit{CalTech256} respectively. About the MIP method, the first step is to gain target class knowledge with \textit{DeepInversion}~\cite{yin_dreaming_2020}. So, we use $\lambda_0 = 1\times10^{-1},1\times10^{-2},1\times10^{-2}$; $\lambda_1 = 1\times10^{-5},1\times10^{-6},1\times10^{-3}$; $\lambda_2 = 1\times10^{-3},1\times10^{-2},1\times10^{-5}$; $\lambda_3 = 1,1\times10^{-1},1\times10^{-1}$ for \textit{Cifar100}, \textit{TinyImageNet}, and \textit{CalTech256} respectively. And in all MI attacks, we use SGD for optimization with a $1\times10^{-2}$ learning rate and run 5000 epochs. In the next poisoning step, we still use SGD as the optimizer and $\alpha_1 = 1\times10^{-3}$, $\alpha_2 = 1\times10^{-5}$ for each dataset.

\subsubsection{Metrics}
Our metric used the accuracy of the target class and the main task on the training dataset because our attack was launched during training processing. Another metric is the cross-entropy loss on the target class of the training dataset.

\subsubsection{Result}
The result has been illustrated in Table ~\ref{Table1}. We can find that MR models have lower main task accuracy because the adversary collects data from the same distribution rather than identical data. MP and MIP keep higher main task accuracy, but the target class loss is lower than the MR method. In our opinion, we believe the success of our inversion attack depends on the loss gap between the main task and the target class. 

%\begin{table*}
\begin{table}[h]
\Huge
\centering
\caption{Evaluation of Malicious Models}
\label{Table1}
\renewcommand\arraystretch{1.5}
\resizebox{\linewidth}{!}{
\begin{tabular}{ccccc} 
\hline
\multirow{2}{*}{\textbf{Method}}                      & \multirow{2}{*}{\textbf{Metric}} & \multicolumn{3}{c}{\textbf{Datasets}}            \\ 
\cline{3-5}
&       & Cifar100   & TinyImageNet & CalTech256        \\ 
\hline
\multirow{4}{*}{\makecell{Model Retrain \\ (MR)}}               & Target Class Acc.       & 0.00\%     & 0.00\%       & 0.00\%      \\ & Target Class Loss       & 265.912 & 252.011  & 108.718  \\ 
\cline{2-5} & Main Task Acc.          & 87.34\%    & 81.77\%      & 96.13\%     \\
 & Main Task Loss          & 2.989   & 2.189     & 0.541    \\ 
\hline
\multirow{4}{*}{\makecell{Model Poisoning \\ (MP)}}             & Target Class Acc.       & 0.00\%     & 0.00\%       & 0.00\%      \\  & Target Class Loss       & 36.064  & 28.553    & 20.586   \\ 
\cline{2-5} & Main Task Acc.          & 96.90\%    & 99.29\%      & 99.45\%     \\
 & Main Task Loss          & 0.435   & 0.151     & 0.088   \\ 
\hline
\multirow{4}{*}{\makecell{Model 
  Inversion \\ Poisoning \\ (MIP)}} & Target Class Acc.       & 0.00\%     & 0.00\%       & 0.00\%      \\
 & Target Class Loss       & 36.040  & 46.807    & 67.262   \\ 
\cline{2-5} & Main Task Acc.          & 98.97\%    & 98.95\%      & 99.13\%     \\
 & Main Task Loss          & 0.133   & 0.252     & 0.268\\
\hline
\end{tabular}
}
\end{table}
% \end{table*}


\subsection{Model Replacement Evaluation}
In subsection~\ref{section-modelReplacement}, we show the model replacement method for all AGRs.  In this section, we detail how we replace the global model with malicious models in practice. 

\subsubsection{AGR-Selection}
According to our core theory in section~\ref{section-framework}, our method is only available for AGRs that use averaging aggregation in the final step. Thus, we select Multi-krum~\cite{blanchard_machine_2017}, Bulyan~\cite{mhamdi_hidden_2018}, AFA~\cite{cao_fltrust_2022}and Fang~\cite{fang_local_2020}.

\subsubsection{Implement Details} In practice, we focus on FedSGD~\cite{konecny_federated_2016} structure.  Here, we assume each client has independently and identically distributed (I.I.D) datasets. And to reduce the complexity of the experiment, we also assume all clients will attend training in each round. In practice, each client resamples the given training dataset. And around 20\% of clients are malicious, specific settings have also been shown in Table~\ref{Table_ModelRep}.

\subsubsection{Metrics}~\label{subsubsection:modelRepMetrics} In the model replacement process, we focus on the global model target class and main task performance on the training dataset. Thus, we select the accuracy and loss of the main task and target class as important metrics. Then, we also record the beginning and final replacement distances. The distance is based on the $l_2$ distance, and the formula is $\sqrt{\sum^l_{l_0=1}(\phi_1-\phi_2)^2/d_\phi}$ where $l$ represents the number of layers, $\phi$ represents the layer parameters, $d_\phi$ is the parameter dimension. When the final replacement distance is almost zero, we can regard that replacement processing as finished.

\subsubsection{Result} The result has been given in Table~\ref{Table_ModelRep}. Our model replacement method has succeeded in all settings. And almost all final models' metrics are near respective malicious models which showed in Table~\ref{Table1}.  Generally, MR is the most difficult one to replace the global model. And we can find that Fang and AFA are more robust because the target class loss of the final replaced models is lower than the corresponding malicious models. 


\begin{table*}
\centering
\Huge
\caption{Model Replacement Result. The three numbers in setting represent the number of clients, batch size, and the number of
malicious clients.The model distance formula has been defined in section~\ref{subsubsection:modelRepMetrics}.}
\label{Table_ModelRep}
\resizebox{1\linewidth}{0.5\height}{
\begin{tblr}{
  cells = {c},
  cell{1}{1} = {r=2}{},
  cell{1}{2} = {r=2}{},
  cell{1}{3} = {r=2}{},
  cell{1}{4} = {r=2}{},
  cell{1}{5} = {c=6}{},
  cell{3}{1} = {r=15}{},
  cell{3}{2} = {r=5}{},
  cell{8}{2} = {r=5}{},
  cell{13}{2} = {r=5}{},
  cell{18}{1} = {r=15}{},
  cell{18}{2} = {r=5}{},
  cell{23}{2} = {r=5}{},
  cell{28}{2} = {r=5}{},
  cell{33}{1} = {r=15}{},
  cell{33}{2} = {r=5}{},
  cell{38}{2} = {r=5}{},
  cell{43}{2} = {r=5}{},
  vline{2-5,7,9} = {-}{},
  hline{2} = {4-10}{},
  hline{1,3,18,33,48} = {-}{},
  hline{8,13,23,28,38,43} = {2-10}{},
}
Datasets     & Model & AGR        & Setting                         & Metric            &                         &                &                &                              &                        \\
             &       &            &                                 & {Target Class\\ Accuracy} & {Target Class\\ Loss} & {Main Task\\ Accuracy} & {Main Task\\ Loss} & {Initialized Model\\Distance($10^{-3}$)} & {Final Model\\ Distance($10^{-3}$)} \\
Cifar100     & MR    & Standard   & 50x32 10                        & 0.000             & 184.089                 & 87.432         & 2.305          & 2220.763                     & 4.082                  \\
             &       & Multi-Krum & 50x32 10                        & 0.000             & 251.593                 & 87.434         & 2.982          & 2220.763                     & 0.697                  \\
             &       & Bulyan     & 51x32 10                        & 0.000             & 250.050                 & 87.840         & 2.948          & 2220.763                     & 5.406                  \\
             &       & AFA        & 50x32 10                        & 0.000             & 109.734                 & 88.144         & 1.518          & 2220.763                     & 68.587                 \\
             &       & Fang       & 50x32 10                        & 0.000             & 227.848                 & 87.674         & 2.731          & 2220.763                     & 8.033                  \\
             & MP    & Standard   & 40x32 8                         & 0.000             & 27.679                  & 96.522         & 0.359          & 61.046                       & 1.798                  \\
             &       & Multi-Krum & 40x32 8                         & 0.000             & 30.377                  & 95.534         & 0.411          & 61.046                       & 0.473                  \\
             &       & Bulyan     & 41x32 8                         & 0.000             & 30.430                  & 93.816         & 0.457          & 61.046                       & 0.254                  \\
             &       & AFA        & 40x32 8                         & 0.000             & 18.815                  & 97.680         & 0.240          & 61.046                       & 17.086                 \\
             &       & Fang       & 40x32 8                         & 0.000             & 27.401                  & 94.318         & 0.414          & 61.046                       & 4.437                  \\
             & MIP   & Standard   & 50x32 10                        & 0.000             & 30.524                  & 98.978         & 0.306          & 1087.533                     & 2.823                  \\
             &       & Multi-Krum & 50x32 10                        & 0.000             & 34.375                  & 98.976         & 0.345          & 1087.533                     & 0.018                  \\
             &       & Bulyan     & 51x32 10                        & 0.000             & 29.263                  & 98.980         & 0.293          & 1087.533                     & 45.807                 \\
             &       & AFA        & 50x32 10                        & 0.000             & 30.887                  & 98.978         & 0.310          & 1087.533                     & 2.427                  \\
             &       & Fang       & 50x32 10                        & 0.000             & 30.221                  & 98.978         & 0.303          & 1087.533                     & 2.958                  \\
TinyImageNet & MR    & Standard   & 40x32 8                         & 0.000             & 225.292                 & 81.721         & 2.072          & 1237.702                     & 1.839                  \\
             &       & Multi-Krum & 40x32 8                         & 0.000             & 258.418                 & 81.718         & 2.235          & 1237.702                     & 1.245                  \\
             &       & Bulyan     & 41x32 8                         & 0.000             & 260.655                 & 79.663         & 2.395          & 1237.702                     & 0.813                  \\
             &       & AFA        & 40x32 8                         & 0.000             & 257.342                 & 81.716         & 2.233          & 1237.702                     & 0.278                  \\
             &       & Fang       & 40x32 8                         & 0.000             & 122.856                 & 80.770         & 1.636          & 1237.702                     & 7.397                  \\
             & MP    & Standard   & 30x32 6                         & 0.000             & 27.227                  & 99.335         & 0.142          & 89.778                       & 1.025                  \\
             &       & Multi-Krum & 30x32 6                         & 0.000             & 28.284                  & 99.285         & 0.149          & 89.778                       & 0.078                  \\
             &       & Bulyan     & 31x32 6                         & 0.000             & 27.789                  & 99.333         & 0.145          & 89.778                       & 2.044                  \\
             &       & AFA        & 30x32 6                         & 0.000             & 27.024                  & 99.323         & 0.141          & 89.778                       & 0.625                  \\
             &       & Fang       & 30x32 6                         & 0.000             & 28.174                  & 99.310         & 0.147          & 89.778                       & 0.544                  \\
             & MIP   & Standard   & 40x32 8                         & 0.000             & 44.799                  & 99.260         & 0.233          & 128.167                      & 1.367                  \\
             &       & Multi-Krum & 40x32 8                         & 0.000             & 45.790                  & 99.151         & 0.241          & 128.167                      & 0.263                  \\
             &       & Bulyan     & 41x32 8                         & 0.000             & 45.177                  & 99.330         & 0.232          & 128.167                      & 1.878                  \\
             &       & AFA        & 40x32 8                         & 0.000             & 36.747                  & 99.459         & 0.186          & 128.167                      & 21.990                 \\
             &       & Fang       & 40x32 8                         & 0.000             & 41.507                  & 99.367         & 0.213          & 128.167                      & 2.622                  \\
CalTech256   & MR    & Standard   & 10x8 2                          & 0.000             & 114.571                 & 96.072         & 0.569          & 288.970                      & 2.448                  \\
             &       & Multi-Krum & 10x8 2                          & 0.000             & 136.099                 & 95.831         & 0.679          & 288.970                      & 43.910                 \\
             &       & Bulyan     & 11x8 2                          & 0.000             & 118.328                 & 96.050         & 0.581          & 288.970                      & 9.523                  \\
             &       & AFA        & 10x8 2                          & 0.000             & 94.622                  & 63.851         & 1.862          & 288.970                      & 195.884                \\
             &       & Fang       & 10x8 2                          & 0.000             & 39.601                  & 91.178         & 0.490          & 288.970                      & 174.439                \\
             & MP    & Standard   & 10x8 2                          & 0.000             & 20.364                  & 99.477         & 0.083          & 40.019                       & 4.474                  \\
             &       & Multi-Krum & 10x8 2                          & 0.000             & 20.528                  & 99.460         & 0.087          & 40.019                       & 0.603                  \\
             &       & Bulyan     & 11x8 2                          & 0.000             & 20.561                  & 99.452         & 0.088          & 40.019                       & 0.857                  \\
             &       & AFA        & 10x8 2                          & 0.000             & 25.588                  & 98.672         & 0.133          & 40.019                       & 11.968                 \\
             &       & Fang       & 10x8 2                          & 0.000             & 20.377                  & 99.469         & 0.086          & 40.019                       & 1.603                  \\
             & MIP   & Standard   & 10x8 2                          & 0.000             & 70.446                  & 99.444         & 0.263          & 217.541                      & 6.819                  \\
             &       & Multi-Krum & 10x8 2                          & 0.000             & 67.188                  & 99.186         & 0.265          & 217.541                      & 0.718                  \\
             &       & Bulyan     & 11x8 2                          & 0.000             & 70.383                  & 99.351         & 0.269          & 217.541                      & 9.314                  \\
             &       & AFA        & 10x8 2                          & 0.000             & 71.169                  & 98.849         & 0.291          & 217.541                      & 11.477                 \\
             &       & Fang       & 10x8 2                          & 0.000             & 48.784                  & 99.540         & 0.180          & 217.541                      & 22.017                 
\end{tblr}
}
\end{table*}


\subsection{Targeted Inversion Attack Evaluation}
The final step is to monitor gradients and invert target class images continuously. 

\subsubsection{Implement Details} In this step, we follow the federated learning framework setting in the model replacement part. According to \ref{section-gradientInversion}, the adversary needs to invert aggregated gradient in each round. But to control the inversion probability and improve experiment efficiency, we manually confirm the input under effective inversion conditions. After inferring the aggregated gradient, we set $\lambda_0 = 1\times10^{-1}$; $\lambda_1 = 1\times10^{-2}$; $\lambda_2 = 1\times10^{-6}$; $\lambda_3 = 1.0$ for 
in the final inversion step.

\subsubsection{Metrics} To evaluate inverse image quality and similarity, we choose three indicators: i) the peak signal-to-noise ratio (PSNR)  ii) the learned perceptual image patch similarity (LPIPS)~\cite{zhang2018unreasonable}, and 
iii) the structural similarity index measure (SSIM)~\cite{wang2004image}.

\subsubsection{Result} The inversion result has been illustrated in Table \ref{Table_InversionResult}. Though the inverse image contains some noise, the important semantic features still have been disclosed under our attack.
% \begin{figure*}[]
% \centering
% \includegraphics[width=1\textwidth]{Figure/Batch_Effect_Image.jpg}
% \caption{Inverse images under different settings. We applied PSNR, LPIPS, and SSIM as metrics}
% \label{Fig_BatchEffect}
% \end{figure*}

% \begin{figure*}[!t]
% 	\centering
% 	\subfloat[CTGI on Cifar100 Inversion Result]{\includegraphics[width=1\textwidth]{Figure/InversionResult/Cifar100InversionResult.jpg}%
% 		\label{Fig_InversionResultSubCifar}}
% 	\hfil
% 	\subfloat[CTGI on TinyImageNet Inversion Result]{\includegraphics[width=1\textwidth]{Figure/InversionResult/TinyImageNetInversionResult.jpg}%
% 		\label{Fig_InversionResultSubImageNet}}
%     \hfil
% 	\subfloat[CTGI on CalTech256 Inversion Result]{\includegraphics[width=1\textwidth]{Figure/InversionResult/CalTech256InversionResult.jpg}%
% 		\label{Fig_InversionResultSubCalTech}}
% 	\caption{Inversion Result. The three numbers under each AGR represent the number of clients, batch size, and the number of malicious clients. PSNR, LPIPS, and SSIM are used as metrics.}
% 	\label{Fig_InversionResult}
% \end{figure*}


\begin{figure*}[!t]
	\centering
	\subfloat[CTGI on Cifar100 Inversion Result]{\includegraphics[width=1\textwidth]{Figure/InversionResult/IR-Cifar100.pdf}%
		\label{Fig_InversionResultSubCifar}}
	\hfil
	\subfloat[CTGI on TinyImageNet Inversion Result]{\includegraphics[width=1\textwidth]{Figure/InversionResult/IR-TinyImageNet.pdf}%
		\label{Fig_InversionResultSubImageNet}}
    \hfil
	\subfloat[CTGI on CalTech256 Inversion Result]{\includegraphics[width=1\textwidth]{Figure/InversionResult/IR-CalTech256.pdf}%
		\label{Fig_InversionResultSubCalTech}}
	\caption{Inversion Result. The three numbers under each AGR represent the number of clients, batch size, and the number of malicious clients. PSNR, LPIPS, and SSIM are used as metrics.}
	\label{Fig_InversionResult}
\end{figure*}



==> chapters/intro.tex <==
\section{Introduction}
Federated Learning (FL)~\cite{mcmahan_communication-efficient_2017,konecny_federated_2016,shokri_privacy-preserving_2015} is an emerging distributed learning framework. It encourages more clients or participants (e.g., private mobile devices or IoT devices) to join the federated training and improve model generalization without sharing their private data. Especially, multiple clients can train the distributed model on their private datasets locally and submit the local model or gradient to the server, then the server will aggregate these updates using an aggregation algorithm (AGR). 


However, due to the distributed feature, FL is vulnerable to various attacks. An adversary can submit malicious updates and gain the global model or gradients used for adversarial operations based on the adversary's goal. Common attacks include: i) \textit{Inference attack}~\cite{nasr_comprehensive_2019,melis_exploiting_2019}, which tends to infer private dataset membership or property; ii) \textit{Poisoning attack}~\cite{blanchard_machine_2017,fang_local_2020,baruch_little_2019,shejwalkar_manipulating_2021}, in which the adversary tries to manipulate model performance to cause a denial of service (DoS) or mount a backdoor; iii) \textit{Inversion Attack}~\cite{fredrikson_model_2015,zhu_deep_2019,geiping_inverting_2020,yin_dreaming_2020,yin_see_2021,zhao_idlg_2020,wen_fishing_2022,fowl_robbing_2022,boenisch_when_2021,jeon_gradient_2021,usynin_beyond_2022,karras_analyzing_2020,ye_label-only_2022}, which includes model inversion attack (MIA) and gradient inversion attack (GIA). Generally, the adversary will try to reconstruct other user data from gradient or model. Typical model inversion attack~\cite{fredrikson_model_2015} attempts to fit real confidence score distribution to extract training data from neural networks based on black-box access. More advanced model inversion attack can only use label~\cite{kahla_label-only_2022} or exploit GAN~\cite{struppek_plug_2022} to launch attack. Then, in the gradient attack, the attacker optimizes random noise to approach the real gradient and reconstruct input data. We focus on the gradient inversion attack in our paper because the gradient inversion attack can directly gain other client data, which breaks the most important privacy norm of FL. 

% \jiaheng{We investigate state-of-the-art GIAs and find potential risks if attackers can break some limitations.}

% \lyz{There is a gap between Inversion Attack (contains GIA and model inversion) and the below gradient inversion attack. need to add 1-2 sentences to clarify further.}

Currently, existing gradient inversion attacks (GIAs) suffer from some or all limitations listed below: 
\begin{itemize}
    \item The adversary must control the server.  Many inversion attack methods require server control to launch the attack, like these proposed attacks~\cite{geiping_inverting_2020,yin_see_2021,wen_fishing_2022,fowl_robbing_2022,boenisch_when_2021}. But in the real world, the server is the hardest entity to be controlled in any FL system.
    \item Label inference affects inversion attack efficiency. Label inference, which was firstly demonstrated by DLG~\cite{zhu_deep_2019} through optimization and then improved by iDLG~\cite{zhao_idlg_2020}, which can analytically recover labels based on the gradient.
    It determines the successful possibility of inversion attack. And GradInversion~\cite{yin_see_2021} found it difficult to infer entire batch labels if the batch contains the same label.
    \item Inversion attacks require strong prior knowledge. Like GradInversion~\cite{yin_see_2021}, the inversion attack needs batch normalization information. And methods based on generative methods~\cite {jeon_gradient_2021,usynin_beyond_2022,karras_analyzing_2020} require distribution of the training data as the prior for the adversary.
    \item The adversary has to change the model structure or parameters. Some methods need the adversary to trap clients~\cite{boenisch_when_2021,wen_fishing_2022} into a predefined status that the adversary flavors, which may break main task performance or change the entire training framework~\cite{fowl_robbing_2022}.
\end{itemize}

{\iffalse
In the practical FL scenario, the server usually belongs to trusted entities or is under strong supervision. But clients generally are private devices and perhaps in large quantities. Securing all clients is expensive and impossible, so we discover potential risks: is it possible to impose the inversion attack as a client? In normal FL training, clients can get the aggregated gradient of the previous round by calculating the differences of global model weights, but the aggregated gradient may contain immeasurable data samples' key features. To reconstruct all samples is very hard and there is no effective label inference method in such scenario~\cite{zhu_deep_2019,zhao_idlg_2020,geiping_inverting_2020,yin_see_2021}. However, if the adversary focuses on a targeted class, he/she needs not to invert all samples and infer labels (directly use the targeted class label). Now, the biggest question is how to draw the targeted samples' gradient from the aggregated gradient. In this work, we denote the targeted samples' gradient as the \textit{targeted gradient}. An easy way is to scale up the targeted gradient and make it distinct in the aggregated gradient. So if required to change the aggregated gradient, the adversary needs to replace the global model with a crafted malicious model to achieve this. The replacement process can be regarded as a model poisoning attack. Finally, to put all ideas together and summarize them: the adversary needs to craft a malicious model first which can magnify the targeted gradient and then replace the global model with it. Next, the adversary can obtain the targeted gradient from the aggregated gradient and try to invert it.

To implement our assumption, in this work, we propose a client-side targeted gradient inversion attack (\attack). As Figure~\ref{fig:overview} demonstrated, our attack framework mainly contains three steps: i) crafting a malicious model; ii) replacing the global model; iii) inverting targeted gradients. \fi}

To overcome these challenges, in this work, we propose a client-side targeted gradient inversion attack (\attack). As Figure~\ref{fig:overview} demonstrated, our attack framework mainly contains three steps: i) crafting a malicious model; ii) replacing the global model; iii) inverting targeted gradients. 

In the first step, the adversary intends to craft a malicious model which can magnify the targeted gradient. According to the gradient formula, the malicious model bases increasing loss variance to make the targeted gradient distinct from the aggregated gradient, thus actually the malicious model is a targeted poisoning model. We provide three methods to craft malicious models depending on the adversary's knowledge level. Then the next step is model poisoning. But in FL, the server generally equips Byzantine-robust
AGRs~\cite{blanchard_machine_2017,mhamdi_hidden_2018,cao_fltrust_2022,fang_local_2020,xie_generalized_2018,yin_byzantine-robust_2018}. Robust AGRs are useful defense methods to filter malicious updates based on the performance of validation dataset~\cite{cao_fltrust_2022,fang_local_2020}, non-averaging aggregation~\cite{xie_generalized_2018,yin_byzantine-robust_2018} or updates distribution~\cite{blanchard_machine_2017,mhamdi_hidden_2018}. Considering the existing AGRs, we design an effective method to optimize the malicious update as a disguised benign update by mixing the benign update and the malicious replacement vector. And the adversary can adjust the mixing hyper-parameters to speed up poisoning or make the update more sneaky against AGR. When the malicious update has been regarded as a benign update by AGR and injected into the global model, the update intends to mislead the global model and make it approach the crafted malicious model. If any client receives the poisoning global model and trains targeted samples on it, the produced gradient will be very distinct and the adversary can obtain it from the aggregated gradient. Finally, the adversary can launch the gradient inversion attack on the targeted gradient. In this step, we combine advanced gradient inversion methods and mainly reference IG~\cite{geiping_inverting_2020} and GradInversion~\cite{yin_see_2021}.

Compared to existing gradient attacks, our attack can effectively launch an attack from the client side and does not require more knowledge or special model structures. And because \attack is targeted,  inverting the targeted samples that belong to other clients is easier than inverting an entire batch of samples. Moreover, \attack does not need batch normalization layer information~\cite{yin_see_2021} and accurate label inference~\cite{zhao_idlg_2020}. Then \attack preserves main task performance while avoiding any modification to the general training framework~\cite{wen_fishing_2022} to stealthy invert targeted sample's gradients.

% Our attack can effectively launch an attack from the client side and does not require more knowledge or special model structures. The basic idea of \attack is to make the gradient associated with the target sample more distinct than other samples' gradients. Correspondingly, inverting the target sample that belongs to other clients is easier than inverting an entire batch of samples. \attack does not need batch normalization layer information~\cite{yin_see_2021} and accurate label inference~\cite{zhao_idlg_2020}. Besides, \attack preserves main task performance while avoiding any modification to the general training framework~\cite{wen_fishing_2022} to stealthy invert targeted sample's gradients.  \yanjun{We need some insights here} These steps will be explained in the next sections.

The contributions of our work are summarized as follows:
\begin{itemize}
    \item We proposed a new client-side targeted gradient inversion attack that can launch attacks from the client side which is more threatening than attacks that require server control.
    \item Our attack is stealthy, the adversary can follow the general training framework and maintain normal main task performance. And it is built upon fewer assumptions of the adversary, e.g., it does not require known data distribution as a prior or accurate label inference.
    \item We instantiated the concept of client-side gradient inversion attack by taking advantage of wisdom from existing attacks, including IG~\cite{geiping_inverting_2020}, DeepInversion~\cite{yin_dreaming_2020}, Model Poisoning~\cite{shejwalkar_manipulating_2021} and so on. This may inspire the community to consider that mixed attacks may damage FL more seriously than any single attack.
\end{itemize}
